V-Cloak: Intelligibility-, Naturalness- & Timbre-Preserving Real-Time Voice Anonymization

Voice data generated on instant messaging or social media applications contains unique user voiceprints that may be abused by malicious adversaries for identity inference or identity theft. Existing voice anonymization techniques, e.g., signal processing and voice conversion/synthesis, suffer from degradation of perceptual quality. In this paper, we develop a voice anonymization system, named V-Cloak, which attains real-time voice anonymization while preserving the intelligibility, naturalness and timbre of the audio. Our designed anonymizer features a one-shot generative model that modulates the features of the original audio at different frequency levels. We train the anonymizer with a carefully-designed loss function. Apart from the anonymity loss, we further incorporate the intelligibility loss and the psychoacoustics-based naturalness loss. The anonymizer can realize untargeted and targeted anonymization to achieve the anonymity goals of unidentifiability and unlinkability. We have conducted extensive experiments on four datasets, i.e., LibriSpeech (English), AISHELL (Chinese), CommonVoice (French) and CommonVoice (Italian), five Automatic Speaker Verification (ASV) systems (including two DNN-based, two statistical and one commercial ASV), and eleven Automatic Speech Recognition (ASR) systems (for different languages). Experiment results confirm that V-Cloak outperforms five baselines in terms of anonymity performance. We also demonstrate that V-Cloak trained only on the VoxCeleb1 dataset against ECAPA-TDNN ASV and DeepSpeech2 ASR has transferable anonymity against other ASVs and cross-language intelligibility for other ASRs. Furthermore, we verify the robustness of V-Cloak against various de-noising techniques and adaptive attacks. Hopefully, V-Cloak may provide a cloak for us in a prism world.

==> tables/A2.tex <==
\begin{table*}\centering
\begin{threeparttable}[tt]
% \renewcommand{\TPTminimum}{\linewidth}
\setlength{\abovecaptionskip}{5pt}% 
\setlength{\belowcaptionskip}{0pt}%

\caption{\blue{The performance under different de-noising methods from A2. (TO BE REMOVED)}}

\scriptsize
\setlength{\tabcolsep}{2mm}{
\begin{tabular}{cl|c|rrr|rrr|rrr|rrr|rrr}
\hline
\multicolumn{2}{c|}{\multirow{2}{*}{\textbf{Model}}} & \multicolumn{1}{c|}{\textbf{B0 (\%)}}  & \multicolumn{3}{c|}{\textbf{Mean-Raw (\%)}}                                                                  & \multicolumn{3}{c|}{\textbf{Mean-Cloaked (\%)}}                                                              & \multicolumn{3}{c|}{\textbf{MP3-Raw (\%)}}                                                                   & \multicolumn{3}{c|}{\textbf{MP3-Cloaked (\%)}}                                                               & \multicolumn{3}{c}{\textbf{Quan8-RAW (\%)}}                                                                 \\
\multicolumn{2}{c|}{}                                & \multicolumn{1}{c|}{\textbf{EER}} & \multicolumn{1}{c}{\textbf{MMR}} & \multicolumn{1}{c}{\textbf{WMR}} & \multicolumn{1}{c|}{\textbf{EER}} & \multicolumn{1}{c}{\textbf{MMR}} & \multicolumn{1}{c}{\textbf{WMR}} & \multicolumn{1}{c|}{\textbf{EER}} & \multicolumn{1}{c}{\textbf{MMR}} & \multicolumn{1}{c}{\textbf{WMR}} & \multicolumn{1}{c|}{\textbf{EER}} & \multicolumn{1}{c}{\textbf{MMR}} & \multicolumn{1}{c}{\textbf{WMR}} & \multicolumn{1}{c|}{\textbf{EER}} & \multicolumn{1}{c}{\textbf{MMR}} & \multicolumn{1}{c}{\textbf{WMR}} & \multicolumn{1}{c}{\textbf{EER}} \\ \hline
\multirow{6}{*}{\textbf{ASV}}     & \textbf{EP}     & 0.70                              & 0.61                             & 1.07                             & 0.73                              & 99.85                            & 1.07                             & 57.02                             & 0.46                             & 1.07                             & 0.73                              & 93.86                            & 1.07                             & 32.10                             & 0.88                             & 1.07                             & 0.92                             \\
                                   & \textbf{XV}     & 6.53                              & 6.18                             & 6.87                             & 6.37                              & 97.63                            & 6.91                             & 38.87                             & 5.46                             & 6.91                             & 5.86                              & 88.02                            & 6.87                             & 30.25                             & 11.49                            & 6.91                             & 9.50                             \\
                                   & \textbf{GMM}    & 11.39                             & 12.52                            & 13.00                            & 12.73                             & 79.55                            & 13.00                            & 39.30                             & 12.19                            & 13.00                            & 12.52                             & 76.45                            & 13.00                            & 35.87                             & 15.12                            & 13.00                            & 13.88                            \\
                                   & \textbf{IV}     & 6.03                              & 5.45                             & 4.70                             & 4.90                              & 92.02                            & 4.70                             & 37.91                             & 5.45                             & 4.70                             & 5.11                              & 86.24                            & 4.70                             & 32.25                             & 5.58                             & 4.70                             & 5.12                             \\
                                   & \textbf{IF}     & 9.44                              & 12.60                            & 6.49                             & 10.44                             & 97.67                            & 6.49                             & 47.21                             & 10.04                            & 6.15                             & 8.97                              & 97.17                            & 5.84                             & 44.59                             & 11.83                            & 6.41                             & 10.10                            \\
                                   & \textbf{AVG}    & 6.82                              & 7.47                             & 6.43                             & 7.03                              & 93.34                            & 6.43                             & 44.06                             & 6.72                             & 6.36                             & 6.64                              & 88.35                            & 6.30                             & 35.01                             & 8.98                             & 6.42                             & 7.90                             \\ \hline\hline
\multicolumn{2}{c|}{\multirow{2}{*}{\textbf{Model}}} & \multicolumn{1}{c|}{\textbf{B0 (\%)}}  & \multicolumn{3}{c|}{\textbf{Squz.8-Raw (\%)}}                                                                & \multicolumn{3}{c|}{\textbf{Squz.8-Cloaked (\%)}}                                                            & \multicolumn{3}{c|}{\textbf{Med-Raw (\%)}}                                                                   & \multicolumn{3}{c|}{\textbf{Med-Cloaked (\%)}}                                                               & \multicolumn{3}{c}{\textbf{Quan8-Cloaked (\%)}}                                                             \\
\multicolumn{2}{c|}{}                                & \multicolumn{1}{c|}{\textbf{EER}} & \multicolumn{1}{c}{\textbf{MMR}} & \multicolumn{1}{c}{\textbf{WMR}} & \multicolumn{1}{c|}{\textbf{EER}} & \multicolumn{1}{c}{\textbf{MMR}} & \multicolumn{1}{c}{\textbf{WMR}} & \multicolumn{1}{c|}{\textbf{EER}} & \multicolumn{1}{c}{\textbf{MMR}} & \multicolumn{1}{c}{\textbf{WMR}} & \multicolumn{1}{c|}{\textbf{EER}} & \multicolumn{1}{c}{\textbf{MMR}} & \multicolumn{1}{c}{\textbf{WMR}} & \multicolumn{1}{c|}{\textbf{EER}} & \multicolumn{1}{c}{\textbf{MMR}} & \multicolumn{1}{c}{\textbf{WMR}} & \multicolumn{1}{c}{\textbf{EER}} \\ \hline
\multirow{6}{*}{\textbf{ASV}}     & \textbf{EP}     & 0.70                              & 0.65                             & 1.07                             & 0.80                              & 99.62                            & 1.07                             & 49.58                             & 1.91                             & 1.07                             & 1.49                              & 93.59                            & 1.07                             & 30.46                             & 96.95                            & 1.07                             & 39.12                            \\
                                   & \textbf{XV}     & 6.53                              & 6.57                             & 6.91                             & 6.64                              & 90.76                            & 6.87                             & 33.28                             & 18.28                            & 6.87                             & 12.63                             & 96.64                            & 6.87                             & 38.84                             & 93.89                            & 6.87                             & 31.95                            \\
                                   & \textbf{GMM}    & 11.39                             & 11.53                            & 13.00                            & 12.34                             & 76.12                            & 13.00                            & 35.63                             & 25.54                            & 13.00                            & 18.27                             & 87.36                            & 13.00                            & 47.35                             & 81.12                            & 13.00                            & 41.34                            \\
                                   & \textbf{IV}     & 6.03                              & 5.33                             & 4.70                             & 4.97                              & 88.14                            & 4.70                             & 35.59                             & 15.45                            & 4.70                             & 9.25                              & 87.77                            & 4.70                             & 32.43                             & 79.67                            & 4.70                             & 41.34                            \\
                                   & \textbf{IF}     & 9.44                              & 12.06                            & 6.30                             & 9.98                              & 97.56                            & 6.53                             & 46.66                             & 39.40                            & 6.68                             & 21.89                             & 100                           & 6.60                             & 69.67                             & 90.99                            & 6.49                             & 41.97                            \\
                                   & \textbf{AVG}    & 6.82                              & 7.23                             & 6.40                             & 6.95                              & 90.44                            & 6.43                             & 40.15                             & 20.12                            & 6.46                             & 12.71                             & 93.07                            & 6.45                             & 43.75                             & 88.52                            & 6.43                             & 39.14                            \\ \hline
\end{tabular}}


% \begin{tablenotes}[flushleft]
% \item[] \vspace{-1pt}\hspace{-2pt}\footnotesize Note that $\epsilon=0.1$ in both cases.
% \end{tablenotes}

\label{tab:A2}
\end{threeparttable}
\end{table*}

==> tables/A3.tex <==
\begin{table}\centering
\begin{threeparttable}[t]
% \renewcommand{\TPTminimum}{\linewidth}
\setlength{\abovecaptionskip}{5pt}% 
\setlength{\belowcaptionskip}{0pt}%

\caption{\blue{The performance under adaptive attacker A3.}}

\footnotesize
\setlength{\tabcolsep}{1.2mm}{
\begin{tabular}{@{}l|l|rrr@{}}
\toprule
\textbf{Anon.}       & \textbf{Adversary} & \textbf{MMR (\%)} & \textbf{WMR (\%)} & \textbf{EER (\%)} \\ \midrule
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Untargeted\\ ($\epsilon=0.1$)\end{tabular}} & A1                    & 94.02        & 6.43         & 46.10        \\
& A3                    & 0.03         & 99.67        & 24.38        \\ \midrule
\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Targeted\\ ($\epsilon=0.1$)\end{tabular}}   & A1                    & 98.97        & 4.23         & 52.28        \\
  & A3: w/ key$^\dagger$           & 95.10        & 1.78         & 43.95        \\
  & A3: w/o key$^\dagger$           & 0.01         & 99.99        & 33.29        \\ \bottomrule
\end{tabular}}


\begin{tablenotes}[flushleft]
\item[] \vspace{-1pt}\hspace{-2pt}\footnotesize  $^\dagger$: w/ or w/o key means that the voiceprint of the target speaker is known or unknown to the adversary.
\end{tablenotes}

\label{tab:A3}
\end{threeparttable}
\end{table}


==> tables/population.tex <==
\begin{table*}\centering
\begin{threeparttable}[tt]
% \renewcommand{\TPTminimum}{\linewidth}
\setlength{\abovecaptionskip}{5pt}% 
\setlength{\belowcaptionskip}{0pt}%

\caption{{Evaluation with different population size.}}

\scriptsize
\setlength{\tabcolsep}{2mm}{
\begin{tabular}{cl|c|crr|crr|crr|crr}
\hline
\multicolumn{2}{c|}{\multirow{2}{*}{\textbf{Model}}} & \textbf{B0 (\%)}  & \multicolumn{3}{c|}{\textbf{10 speakers (\%)}}                                                    & \multicolumn{3}{c|}{\textbf{20 speakers (\%)}}                                                    & \multicolumn{3}{c|}{\textbf{30 speakers (\%)}}                                                    & \multicolumn{3}{c}{\textbf{40 speakers (\%)}}                                                                 \\
\multicolumn{2}{c|}{}                                & \textbf{EER} & \textbf{MMR}               & \multicolumn{1}{c}{\textbf{WMR}} & \multicolumn{1}{c|}{\textbf{EER}} & \textbf{MMR}              & \multicolumn{1}{c}{\textbf{WMR}} & \multicolumn{1}{c|}{\textbf{EER}} & \textbf{MMR}              & \multicolumn{1}{c}{\textbf{WMR}} & \multicolumn{1}{c|}{\textbf{EER}} & \textbf{MMR}               & \multicolumn{1}{c}{\textbf{WMR}} & \multicolumn{1}{c}{\textbf{EER}} \\ \hline
\multirow{6}{*}{\textbf{ASV}}      & \textbf{EP}     & 0.70        & 100.0     & 0.85                             & 71.07                             & 100.0   & 0.77                            & 69.50                            & 100.0   & 1.38                           & 70.94                           & 100.0    & 1.49                            & 72.10                                      \\
                                   & \textbf{XV}     & 6.53        & 100.0     & 0.00                             & 47.38                             & 100.0   & 0.00                            & 43.40                            & 100.0   & 0.00                           & 43.68                           & 100.0    & 0.00                            & 44.01                                      \\
                                   & \textbf{GMM}    & 11.39       & 86.14     & 10.80                            & 40.93                             & 83.26   & 10.85                           & 39.75                            & 84.53   & 9.87                           & 41.94                           & 87.89    & 11.38                           & 41.17                                      \\
                                   & \textbf{IV}     & 6.03        & 94.09     & 2.10                             & 29.20                             & 84.85   & 2.60                            & 34.92                            & 87.88   & 3.73                           & 33.97                           & 86.81    & 6.03                            & 37.75                                      \\
                                   & \textbf{IF}     & 9.44        & 96.45     & 15.06                            & 49.07                             & 97.99   & 7.80                            & 47.01                            & 97.55   & 7.65                           & 46.16                           & 97.02    & 6.79                            & 47.22                                      \\\hline
                                   & \textbf{AVG}    & 6.82        & 95.34     & 5.76                             & 47.53                             & 93.22   & 4.40                            & 46.91                            & 93.99   & 4.53                           & 47.34                           & 94.34    & 5.14                            & 48.45                                      \\ 
                                   & \textbf{WCS}    & -           & 86.14     & 0.00                             & 29.20                             & 83.26   & 0.00                            & 34.92                            & 84.53   & 0.00                           & 33.97                           & 86.81    & 0.00                            & 37.75                                      \\ \hline
\end{tabular}}


\begin{tablenotes}[flushleft]
\item[] \vspace{-1pt}\hspace{-2pt}\footnotesize \textbf{AVG}: the average-case scenario, \textbf{WCS}: the worst-case scenario. \textbf{EP}: ECAPA-TDNN, \textbf{XV}: X-vector, \textbf{GMM}: GMM-UBM, \textbf{IV}: ivector-PLDA, \textbf{IF}: iFlytek.
\end{tablenotes}

\label{tab:population}
\end{threeparttable}
\end{table*}
